Assessing the Solvency of Virtual Asset Service Providers: Are Current Standards Sufficient?

Entities like centralized cryptocurrency exchanges fall under the business category of virtual asset service providers (VASPs). As any other enterprise, they can become insolvent. VASPs enable the exchange, custody, and transfer of cryptoassets organized in wallets across distributed ledger technologies (DLTs). Despite the public availability of DLT transactions, the cryptoasset holdings of VASPs are not yet subject to systematic auditing procedures. In this paper, we propose an approach to assess the solvency of a VASP by cross-referencing data from three distinct sources: cryptoasset wallets, balance sheets from the commercial register, and data from supervisory entities. We investigate 24 VASPs registered with the Financial Market Authority in Austria and provide regulatory data insights such as who are the customers and where do they come from. Their yearly incoming and outgoing transaction volume amount to 2 billion EUR for around 1.8 million users. We describe what financial services they provide and find that they are most similar to traditional intermediaries such as brokers, money exchanges, and funds, rather than banks. Next, we empirically measure DLT transaction flows of four VASPs and compare their cryptoasset holdings to balance sheet entries. Data are consistent for two VASPs only. This enables us to identify gaps in the data collection and propose strategies to address them. We remark that any entity in charge of auditing requires proof that a VASP actually controls the funds associated with its on-chain wallets. It is also important to report fiat and cryptoasset and liability positions broken down by asset types at a reasonable frequency.

==> sections_original/0_nontech_summary.tex <==
\section*{Non technical summary}


Virtual asset service providers (VASPs) like centralized cryptocurrency exchanges are companies that facilitate financial activity involving virtual assets (VAs, also called cryptoassets), by enabling their exchange for other VAs or fiat currencies, their custody and transfer via cryptoasset wallets, and portfolio management services \citep{fma2021aml,mica2022proposal,FATF2021guidance}. 

Two major incidents that unfolded within the cryptoasset sector in 2022 highlight that the lack of proper accounting and business continuity concepts are a critical aspect of this industry~\citep{zetzscheremaining}.
%
In May, a bank run on the stablecoin Terra, a cryptoasset whose value was supposed to be pegged to the US dollar, contributed to the collapse of the companies Celsius and Voyager, and the hedge fund Three Arrows Capital. In November, the crypto trading platform FTX collapsed and filed for bankruptcy, leading to BlockFi's downfall and bankruptcy consideration for Aax and Genesis  \citep{econ2022ftx}.
%
While VASPs activities involving fiat currencies are audited according to generally accepted accounting principles, cryptoassets are held in pseudo-anonymous wallets across multiple distributed ledgers~\citep{elbahrawy2017evolutionary} and are not yet systematically audited. 
%
However, transactions executed on distributed ledgers such as Bitcoin and Ethereum are public and can be observed, potentially opening new opportunities to enhance and automate the current auditing procedures.

Our paper aims to propose an approach for determining a virtual asset service provider's solvency status by measuring their cryptoasset holdings, to identify the limits of the current auditing and accounting procedures, and to suggest potential improvements. 
%
We investigate 24 VASPs registered with the Financial Market Authority in Austria and cross-reference data from three distinct sources: their cryptoasset wallets, balance sheet data from the commercial register, and information from supervisory entities.

Using information from the Austrian Financial Market Authority (FMA), we describe what cryptoassets VASPs support and what financial services they provide.
%
We find that they typically operate using multiple cryptoassets, such as bitcoin (N = 20), ether (N = 16), and stablecoins (N = 12).
%
Regarding their service offering, we note that the VASPs we analyzed do not provide saving deposits and loans as traditional banks do. Most of them facilitate the exchange of virtual assets for fiat currency (N = 20) or virtual assets (N = 9), and keep them in custody for their customers (N = 15). 
%
By comparing their activity to traditional financial intermediaries, we find that they are most similar to brokers, money exchanges, and funds, rather than banks.

Next, we concentrate the empirical analysis on four VASPs that have published their balance sheets, allowing to compare their cryptoasset holdings on Bitcoin and Ethereum wallets to their balance sheets. Their market share is around 99\% of the total market share; the remaining VASPs are rather small companies. We find that data are consistent for two VASPs only. 

This enables us to identify gaps in the data collection and propose strategies to address them.
%
First, VASPs employ diverse approaches to manage their cryptoasset transfers, making more challenging to identify their cryptoasset holdings; second, even using a dataset containing more than \num{265000000} deanonymized Bitcoin addresses and \num{278244} tagged Ethereum addresses, and having conducted manual transactions with the VASPs investigated, the resulting data only provide a partial view of their holdings; third%, balance sheets are only reported yearly, asset holdings might differ before and after their publication; fourth
, not all VASPs report balance-sheet items for crypto and fiat asset holdings separately, and VASPs may be subsidiaries of larger corporations and operate under multiple jurisdictions. 

We therefore sketch out our vision for a more systematic, reliable, and highly automated assessment of proof of solvency. 
%
On the cryptoasset side, we remark that any entity in charge of auditing requires proof that a VASP actually controls the funds associated with its on-chain wallets. 
%
VASPs should disclose their cryptoasset wallets and provide additional metadata describing the use of these wallets.
%
On the balance sheet side, reporting requirements for a VASP should report fiat and crypto asset and liability positions broken down by asset types at a reasonable frequency.
%
We conclude by discussing how using cryptographic primitives and automation could improve the current assessment process.


\newpage

==> tables/VASPs_agg.tex <==
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcccc}
	\toprule
	 & \multicolumn{3}{c}{CEX} & \\
	 \cmidrule{2-4}
	Financial services & \makecell[c]{ Group 1 \\ ($N = 7$) } %\makecell[l]{Money\\exchange} 
	             & \makecell[c]{ Group 2 \\ ($N = 6$) } %Broker 
	             & \makecell[c]{ Group 3 \\ ($N = 6$) } %Funds 
	             & \makecell[c]{ Group 4 \\ ($N = 2$) } %\makecell[l]{Payment\\processer} 
	             \\
	\midrule
	\makecell[l]{Custody} & \xmark & \checkmark & \checkmark &  \xmark / \checkmark \\
	\makecell[l]{Exchange \\ of money} & \checkmark & \checkmark & \checkmark & \xmark / \checkmark \\
	\makecell[l]{Payment \\ services} & \xmark & \xmark & \xmark & \checkmark \\
	\makecell[l]{Investment} & \xmark & \xmark & \checkmark & \xmark \\
	Trading %\makecell[l]{Endogenous \\ price setting} 
	& \xmark & \xmark / \checkmark & \xmark & \xmark \\
	\makecell[l]{Vending \\ machines} & \xmark / \checkmark & \xmark & \xmark & \xmark \\
	%Trading & & & &  \\
	%Loans & & & & \\
	%Saving deopsits & & & & \\
	\bottomrule
	%\multicolumn{5}{l}{\footnotesize \textit{Note:} This table is based on personal views of the authors. The \xmark \hspace{0.15em} symbol indicates that no VASP in the group offers the service in the corresponding row, while the \checkmark \hspace{0.15em} symbol means that all offer it. When both are present, only some VASPs in the group offer that service.}\\
	%\vspace{0.03cm}
\end{tabular*}
%\floatfoot
\begin{flushleft}
	{\footnotesize \emph{Notes:} The \xmark \hspace{0.15em} symbol indicates that no VASP in the group offers the service in the corresponding row, while the \checkmark \hspace{0.15em} symbol means that all offer it. When both are present, only some VASPs in the group offer the service. This table reports personal views of the authors on VASPs business models, that might deviate from official data.}
\end{flushleft}
